Semantic-based Data Augmentation for Math Word Problems

It's hard for neural MWP solvers to deal with tiny local variances. In MWP task, some local changes conserve the original semantic while the others may totally change the underlying logic. Currently, existing datasets for MWP task contain limited samples which are key for neural models to learn to disambiguate different kinds of local variances in questions and solve the questions correctly. In this paper, we propose a set of novel data augmentation approaches to supplement existing datasets with such data that are augmented with different kinds of local variances, and help to improve the generalization ability of current neural models. New samples are generated by knowledge guided entity replacement, and logic guided problem reorganization. The augmentation approaches are ensured to keep the consistency between the new data and their labels. Experimental results have shown the necessity and the effectiveness of our methods.

==> 6.case_study.tex <==
% analyza samples: baseline correct, augmentation wrong
In this section, we'll analyze the questions that are predicted correctly before the neural models trained with augmented data but are predicted wrongly afterwards. 
For each error case, we search for a most similar question in $D_{train}$ to see whether these problems have occurred during training phase. 
And it turns out that most of the error cases have a nearly the same question in $D_{train}$ as shown in Table \ref{case_study_seq2tree}.
The $Q_{te}\in D_{test}$ are error predicted questions in the testing set. $Q_{tr} \in D_{train}$ are their similar questions found in the training set. %And pred. $Eq$ is the mistaken prediction result after augmentation. 
% As shown in the table, both the textual description and the problem types of the questions in the training set are similar to the error cases.
In the first row of Table \ref{case_study_seq2tree}, the target $Eq$ of the $Q_{tr}$ is $x=n_1\times n_2\div (1+n_3)$. 
% And one of the equation of the augmented samples is $x=(n_4 \times (1+n_3))\div n_2$ as described in \ref{section:logical_augmentation}, which is equivalent to the mistaken predicted equation in template.
According to the logical augmentation described in Sec. \ref{section:logical_augmentation}, one of the $Eq_L$ could be $(\hat{n}\times(1+n_3))\div n_2$, which is equivalent to the mistakenly predicted equation in template.
This result further support our hypothesis in Sec. \ref{section:comparison_results} and explain the performance decreases of complex models on $D_{test}$.
% Considering none of the existing neural MWP solvers have been designed to deal with the local variances, we doubt that they have limited ability to handle the challenging samples in MWP.
% Thus, the introduced challenging samples may hurt the overfitting on the training set leading to the decreases of performances on $D_{test}$. 
% The results on $D_{test}^*$ show that the performances on fresh samples are largely improved with s.based aug., reflecting the improvement of the generalization ability of neural models trained with augmented data.
% It indicates that correctly answering these questions may not reflect the inference and generalization ability of the neural models. 
% The neural models may be overfitting on the training set before augmentation, and the massive challenging samples with only tiny local variances but different labels brought in by the augmentation strategies may break the overfitting on the original training set.

